PSO-PINN: Physics-Informed Neural Networks Trained with Particle Swarm Optimization

Physics-informed neural networks (PINN) have recently emerged as a promising application of deep learning in a wide range of engineering and scientific problems based on partial differential equation (PDE) models. However, evidence shows that PINN training by gradient descent displays pathologies that often prevent convergence when solving PDEs with irregular solutions. In this paper, we propose the use of a particle swarm optimization (PSO) approach to train PINNs. The resulting PSO-PINN algorithm not only mitigates the undesired behaviors of PINNs trained with standard gradient descent but also presents an ensemble approach to PINN that affords the possibility of robust predictions with quantified uncertainty. We also propose PSO-BP-CD (PSO with Back-Propagation and Coefficient Decay), a hybrid PSO variant that combines swarm optimization with gradient descent, putting more weight on the latter as training progresses and the swarm zeros in on a good local optimum. Comprehensive experimental results show that PSO-PINN with the proposed PSO-BP-CD algorithm outperforms PINN ensembles trained with other PSO variants or with pure gradient descent.

==> sections/4_results_OLD.tex <==
\section{Experimental Results}
\label{sec:results}


\begin{figure*}[t]
    \begin{center}
    % \includegraphics[width=1.9\columnwidth]{fig/poisson_train.png} % paper version
    \includegraphics[width=1\columnwidth]{fig/poisson_train.png}    % arXiv Version
    \hfill
    \end{center}
    \caption{
    % 
    \textbf{Poisson Equation} -- First row: solutions in the PSO-PINN ensemble as training progresses. Second row: Best individual, mean and variance of PSO-PINN ensemble. Third row: PSO-PINN mean loss error. The grey band is the two-sided 1-standard deviation region.}
    \label{fig:poisson_train}
\end{figure*}

In this section, we study the performance of PSO-PINN by means of experimental results using several classical ODE and PDE benchmarks. After presenting the solutions of the various equations obtained by PSO-PINN, we discuss possible parametrizations for the algorithm, and finally we compare the PSO-PINN to a pure ensemble of ADAM-trained PINNs, without communication among the PINNs as in PSO-PINN. The main figure of merit used in this section is the $L_2$ error:

\begin{equation}
    L_2 \ \text{error} \,=\, \frac{\sqrt{\sum_{i=1}^{N_U} |\hat{f}(\mathbf{x}_i) - U(\mathbf{x}_i)|^2}}{\sqrt{\sum_{i=1}^{N_U} |U(\mathbf{x}_i) |^2}}\,.
\end{equation}
where $\hat{f}(\mathbf{x})$ is the prediction and $U(\mathbf{x})$ is the analytical solution or a high-fidelity approximation over a test mesh $\{\mathbf{x}_i\}_{i=1}^{N_U}$. All experiments in this section were performed using Tensorflow 2~\cite{tensorflow2015-whitepaper}.

\subsection{Study Case Problems}

\subsubsection{The Poisson Equation}

The first problem is the 1D Poisson equation, which is an ordinary differential equation defined by:
\begin{equation}
    \begin{split}
        &u_{xx} = g(x)\,, \quad x \in [0,1]\,,  \\ 
        &u(0) = a\,,\quad u(1) = b\,.
    \end{split}
\end{equation}
For this example, we manufacture $g(x)$ so that $u(x) = \sin(2\pi x)$, with $u(0) = u(1) = 0$. Since this problem describes an ODE (relatively simpler than a PDE), we may use a relatively shallow architecture. In this case, we are using a network with 3 layers of 10 neurons, trained for only 90 iterations. The particles in the PSO-PINN swarm were initialized using the uniform distribution and the values assigned for $\beta$, $c_1$ and $c_2$ were 0.9, 0.08, and 0.5, respectively.  

Figure \ref{fig:poisson_train} displays the results. We can see that the PSO-PINN swarm finds an excellent approximation to the solution rather quickly, in less than one hundred iterations. Also, the mean and variance show that the entire swarm has good convergence. The variance of the swarm may be interpreted as the uncertainty associated with the approximation. As the swarm approach a consensus we should notice a reduction in the variance of the solution, indicating more confidence in the final result.

\subsubsection{The Advection Equation}
The advection equation models the transport of a substance by bulk motion of a fluid. In this example, we are assuming a linear univariate advection equation~\cite{leveque2002finite}:
\begin{equation}
  q_t + uq_x = 0
  \end{equation}
where $u$ is the constant velocity. The Riemman initial condition is  
\begin{equation}
     q(x,0) = 
        \begin{cases} 
            q_l, & 0 \leq x < x_0 \,, \\
            q_r , & x_0 < x \leq L\,. 
        \end{cases}
  \end{equation}
This simple problem has as solution:
\begin{equation}
     q(x,t) = 
        \begin{cases} 
            q_l, & 0 \leq x < x_0+ut \,, \\
            q_r, & x_0+ut < x \leq L\,,     
        \end{cases}
  \end{equation} 
for $0 \leq t < (L-x_0)/u$. In other words, the initial discontinuity in concentration is simply advected to the left with constant speed $u$.

\begin{figure}
\begin{center}
% \includegraphics[width=1\columnwidth]{fig/advection.png}    % Paper Version
\includegraphics[width=1\columnwidth]{fig/advection.png}  % ArXiv Version
\hfill
\end{center}
\caption{
% 
\textbf{Advection Equation} -- The PSO-PINN solution is the mean value of the results in the swarm. Each column depicts a snapshot of the training process. The first column illustrates the swarm after 100 iterations, the second column shows the swarm after 200 iterations, and finally, the third column represents the swarm after 500 iterations. 
}
\label{fig:advection}
\end{figure}

For this problem we used a PSO-PINN swarm composed of 100 particles, each one with 5 layers of 8 neurons, and trained it through 500 iterations. The PSO attributes $\beta$, $c_1$, and $c_2$ were set to 0.99, 0.008 and 0.05, respectively. Figure \ref{fig:advection} illustrates the training process and shows that PSO-PINN found a good approximation after just 500 iterations, with a good convergence to the true solution. After ten independently training the PSO-PINN, we found the $L_2$ error mean of 3.27E-2 and the mean variance was equal to 2.84E-2.

\subsubsection{The Burgers Equation}

Here we consider the following version of the the viscous Burgers equation:
    \begin{equation}
    \label{eq:burgers}
        \begin{split}
            &\frac{\partial u}{\partial t} + u\frac{\partial u}{\partial x} = \nu\frac{\partial^2u}{\partial x^2}, \qquad x \in [-1, 1], \quad t \in [0, 1] \\
            &u(0,x) = -\sin(\pi x)\,, \\
            &u(t, -1) = u(t,1) = 0\,,
        \end{split}
    \end{equation}
    with $\nu = 0.01/\pi$

For the Burgers equation, we trained a PSO-PINN instance with two input neurons, 8 hidden layers of 10 neurons each, and an output layer of size 1 corresponding to the output of the approximation u(x, t). We used a swarm containing 20 particles (networks), and the algorithm was trained for 2000 iterations with the values of $\beta$, $c_1$, and $c_2$ to 0.9, 0.04 and 0.05, respectively. After 10 consecutive experiments, the mean for the $L_2$ error was 1.25E-2 with an variance of 8.73E-3. The best ensemble the $L_2$ error was 5.79E-3. More details can be found on the Table \ref{tab:model_selection}.

\subsubsection{The Heat Equation}

The 1D Heat equation models the temperature dissipation in one dimension. That would be the case for the dissipation of the temperature in an iron rod, for example. 
\begin{equation}
\label{eq:heat}
    \begin{split}
        &\frac{\partial u}{\partial t}=\alpha \frac{\partial^2u}{\partial x^2}, \qquad
        x \in [-1, 1], \quad t \in [0, 1] \\
        &u(0,t) = u(1,t)=0,\\
        &u(x,0) = \sin \Big(\frac{n\pi x}{L}\Big),\qquad 0<x<L \\
    \end{split}
\end{equation}
where $L=1$ is the length of the bar, $n=1$ is the frequency of the sinusoidal initial conditions. The reference solution is $u(x,t) = e^{\frac{-n ^2\pi ^2 \alpha t}{L^2}}\sin (\frac{n\pi x}{L})$.
The results displayed in Figure \ref{fig:heat} represents a PSO-PINN solution of a network with 8 layers of 20 neurons each. The swarm was composed by 20 particles and it ran over 4000 iterations. We repeated this experiment for ten times and it resulted in a mean $L_2$ error of 5.14E-3 with a variance of 2.13E-3.  
\begin{figure*}[h]
\begin{center}
% \includegraphics[width=2\columnwidth]{fig/heat.png}     % paper Version
\includegraphics[width=1\columnwidth]{fig/heat.png}    % arXiv Version
\hfill
\end{center}
\caption{
% 
\textbf{Heat Equation} --  In the first row is the cross-section PSO-PINN solution for the problem (the mean values of the swarm predictions). The second row shows the results for the entire domain. The last row displays the analytical solution. 
}
\label{fig:heat}
\end{figure*}   
    
    
\subsubsection{The Diffusion Equation}

This example also describes a 1D heat diffusion equation. We are calling this benchmark the diffusion equation for the sake of organization.  The PDE is given by:
    \begin{equation}
    \label{eq:diffusion}
        \begin{split}
            &\frac{\partial u}{\partial t}- \frac{\partial^2u}{\partial x^2}, = 1 + x cos(t) \quad
            x \in [-1, 1], \quad t \in [0, 1] \\
            &\frac{\partial u}{\partial x}\bigg\rvert_{x=0} = \frac{\partial u}{\partial x}\bigg\rvert_{x=1}= sin(t),\\
            &u(x,0) = 1 + cos(2 \pi x) \\
        \end{split}
    \end{equation}
The exact solution is $u(x,t) = 1 + t + e^{-4 \pi^2 t} cos(2\pi x) + x sin(t)$.

For this example we trained a PSO-PINN with 20 particles. Each element is a network with 5 layers of 8 neurons and they were trained for 2000 iterations.The values of $\beta$, $c_1$, and $c_2$ to 0.9, 0.08 and 0.05, respectively. After 10 consecutive experiments, the mean for the $L_2$ error was 2.17E-2 with a variance of 2.35E-4. More details on the Table \ref{tab:model_selection}.
   
\subsubsection{The Allen-Cahn Equation}

The Allen-Cahn reaction-diffusion PDE is typically used to describe phase-field models to simulate the phase separation in a multi-component alloy. The Allen-Cahn equation is described as follows:

\begin{equation}
    \label{eq:allen-cahn}
        \begin{split}
            &\frac{\partial u}{\partial t} = d\frac{\partial^2u}{\partial x^2} + 5(u - u^3), \quad x \in [-1, 1], \quad t \in [0, 1] \\
            &u(x, 0) = x^2\cos(\pi x) \\
            &u(-1, t) = u(1, t) = -1 \\
        \end{split}
\end{equation}

For the simulations on this paper we kept $d = 0.0001$. We used a PSO-PINN swarm of 20 particles, each one representing a neural network with 5 hidden layers and 20 neurons per layer. In this particular example, we added data points in the domain to aid training (this benachmark is notoriously hard for PINNs to solve~\cite{mcclenny2020self}. The dataset is composed of ten evenly spaced points in the $x$ axis extended over the $t$ domain at 200 intervals.


\subsection{Model Selection}
\label{sec:model_selection}

Most meta-heuristics algorithms for optimization, especially in the PSO family, are rather sensitive to their control parameters\cite{leonard2013optimality, harrison2018self}. This peculiarity may turn the parametrization of the algorithm into a challenging task. For this reason, we performed reiterative experiments, using rounds of 10 repetitions for each parametrization, collected and analyzed the results to understand better each parameter's role in the outcome of the PINN.

There was used four of the PDE problems described in the last section as a baseline to analyze the three different models.  We did a grid search over the parameters ($\alpha$, $\beta$, $c_1$, and $c_2$) and initializations aiming to find the best parametrization for each pair problem/model. The hyper-parameters (number of iterations, layers, etc.) were kept fixed over all experiments in order to give a better perspective on the outcomes of the algorithm, especially after changes in the models and initializations. The population of the ensembles was kept fixed at 20 individuals, where each individual was a PINN with 5 layers and 8 neurons per layer trained for 2000 iterations. 

The Table \ref{tab:model_selection} shows the summary of this experiments. We listed the results for each problem described before, using each one of the models presented in section \ref{sec:models}. The two first columns, "Problem" and "Model", are the only columns with fixed values. The following five columns (Initialization, $\alpha$, $\beta$, $c_1$, and $c_2$) on its turn, represent the best parameters for each problem/model. Finally, the last four columns exhibit the results of the given experiment. The median, variance, and minimum values for the $L_2$ Error are the average values after the 10 rounds of tests, and the best column gives us the best particle from the best swarm.   

As shown in the table, the gradient-assisted optimization achieved the best results for all the proposed problems, either using parameters updating(model 3) or not (model 2). Also, we had a consensus for the best value for the $\alpha$ (Adam's learning rate) as 0.001. Despite the values for $\beta$, $c_1$ and $c_2$ were not unanimous among the results, good results are often obtained using 0.99, 0.008 and 0.05, respectively.


%Paper Version:
% \begin{table*}[h]     
\begin{sidewaystable} 
% \begin{table*}
\begin{center}
\caption{ \textbf{Model Selection} -- The following configurations are the result of a grid search over the initialization, $\alpha$, $\beta$, $c_1$, $c_2$ for each model. 
The two first columns, "Problem" and "Model", have fixed values for the problems and models described in the last sections. The following five columns (Initialization, $\alpha$, $\beta$, $c_1$, and $c_2$) display the best parameters found for each problem/model. Finally, the last three columns have the results of the experiments.
}
\label{tab:model_selection}
\begin{tabular}{lccccccccc}
    \hline
    \multirow{2}{*}{Problem}   & \multirow{2}{*}{Model}  & \multirow{2}{*}{Initialization} & \multirow{2}{*}{$\alpha$} & \multirow{2}{*}{$\beta$} & \multirow{2}{*}{$c_1$} & \multirow{2}{*}{$c_2$} & \multicolumn{3}{c}{$L_2$ Error}           \\ \cline{8-10} 
                               &                         &                                 &                           &                          &                        &                       & Mean              & Variance & Min      \\ \hline
    \multirow{3}{*}{Advection} & 1                       & uniform                         & -                         & 0.99                     & 0.08                   & 0.05                  & 7.08E-02          & 2.47E-03 &\textbf{ 2.25E-02} \\
                               & 2                      & uniform                         & 0.001                     & 0.9                      & 0.04                   & 0.5                    & 3.51E-02          & 1.24E-05 & 3.02E-02 \\
                               & 3                      & uniform                         & 0.001                     & 0.99                     & 0.008                  & 0.05                   & \textbf{3.27E-02} & 4.35E-06 & 2.84E-02 \\ \hline
    \multirow{3}{*}{Burgers}   & 1                       & he                              & -                         & 0.99                     & 0.08                   & 0.05                  & 4.54E-01          & 4.59E-03 & 3.22E-01 \\
                               & 2                      & he                              & 0.001                     & 0.9                      & 0.04                   & 0.05                   &1.47E-01           & 5.37E-03 & 5.79E-02 \\
                               & 3                      & he                              & 0.001                     & 0.9                      & 0.04                   & 0.05                    & \textbf{1.25E-02}          &8.73E-03 & \textbf{5.79E-03} \\ \hline
    \multirow{3}{*}{Diffusion} & 1                       & uniform                         & -                         & 0.99                     & 0.008                  & 0.05                  & 4.95E-02          & 3.78E-06 & 4.77E-02 \\
                               & 2                      & uniform                         & 0.001                     & 0.9                      & 0.04                   & 0.5                    & \textbf{1.99E-02} & 2.28E-04 & \textbf{7.15E-03} \\
                               & 3                      & uniform                         & 0.001                     & 0.9                      & 0.08                   & 0.05                   & 2.17E-02          & 2.35E-04 & 1.09E-02 \\ \hline
    \multirow{3}{*}{Heat}      & 1                       & xavier                          & -                         & 0.99                     & 0.008                  & 0.05                  & 2.62E-01          & 2.07E-03 & 1.91E-01 \\
                               & 2                      & he                              & 0.001                     & 0.9                      & 0.04                   & 0.5                    & 6.60E-03          & 7.61E-06 & 3.68E-03 \\
                               & 3                      & lecun                           & 0.001                     & 0.9                      & 0.008                  & 0.5                    & \textbf{5.14E-03} & 2.88E-06 & \textbf{2.13E-03}
    \end{tabular}
\end{center}
\end{sidewaystable}
% \end{table*}




\subsection{Initialization}
\label{sec:initialization}

The initialization of the weights of a Neural Network may have a critical impact on the training process, which often reflects on model performance. One of the most accepted methods for initialization is the Xavier Initialization\cite{glorot2010understanding}, which attempts to keep the same variance across every layer. 
However, although this approach has been vastly used to initialize deep neural networks, it only takes into account a single neural network. 

It is yet to be proven that such initialization could yield a better population for an ensemble of neural nets (especially for a swarm, the current literature suggests the best approach as an evenly dispersed over the search space). During the initialization of a swarm, we want to cover the search space as much as possible\cite{cazzaniga2015impact}, and there is no evidence that such method could expand the search space concerning the whole swarm. This subject was discussed to some extent in \cite{rauf2018training}. 

We did a brief investigation on how different network initialization would affect the swarm behavior. In Table \ref{tab:model_selection}, we can notice that different problems alongside with different parametrizations required distinct initialization methods. Interestingly, uniform initialization seemed to work well for the Advection and the Diffusion problems. The table \ref{tab:init} summarises the results obtained grouping all the parametrizations used for each initialization.  Notice that changes in the initialization are much less sensitive than changes on the parametrization. This leads us to infer that even if the initialization method must have some level of influence on the final predictor, it is smaller than the changes in the parameters, but it is still noticeable in the final predictor. As well as in the case of parametrizations, the ideal initialization may vary depending on the problem and the parameters. However, the uniform initialization showed a consistent performance in all experiments.

\begin{table}
\begin{center}
\caption{ \textbf{Initialization Methods} --  The median of the $L_2$ errors of the predictors for each problem according to the initialization method.}
\label{tab:init}
\begin{tabular}{lcccc}
\hline
Initialization & Advection         & Burgers           & Diffusion         & Heat              \\ \hline
He             & 4.46E-02          & 3.02E-01          & \textbf{4.66E-02} & 1.41E-02          \\
Lecun          & 4.44E-02          & 3.74E-01          & 4.91E-02          & \textbf{1.02E-02} \\
Uniform        & \textbf{4.05E-02} & \textbf{3.19E-01} & 4.70E-02          & 1.84E-02          \\
Xavier         & 4.81E-02          & 3.24E-01          & 4.99E-02          & 2.37E-02         
\end{tabular}
\end{center}
\end{table}






\subsection{Comparison with Traditional Ensembles of PINNs}


In this section we investigate the performance of the PSO-PINN algorithm in three different problems, comparing it to ensembles of ADAM-trained PINNs. In this comparison, to keep the comparison fair, both methods shared the same network topology (5 hidden layers of 8 neurons), number of iterations (2000), number of collocation points (512) and same size of population (20 particles). 

\subsubsection{The Burgers Equation}
Figure \ref{fig:burgers_pop} illustrates the effect of population size on the accuracy of PSO-PINN. The first column represents the solution using a population of twenty particles, the second and third columns show the solution for a hundred and two hundreds, respectively. In all the cases the ensembles were trained for 2000 iterations. Clearly, the results improve with a larger number of particles, especially for PSO-PINN. This is the expected behavior, since we are in fact increasing the exploration of the search space. 

\begin{figure*}
\begin{center}
% \includegraphics[width=2\columnwidth]{fig/burgers_pops.png}    % paper version
\includegraphics[width=1\columnwidth]{fig/burgers_pops.png}    % arXiv Version
\hfill
\end{center}
\caption{
% 
\textbf{Burger Equation} -- PSO-PINN produce the best results. The results for the baseline PINN with gradient descent were repeated across the columns for comparison purposes.
}
\label{fig:burgers_pop}
\end{figure*}


\subsubsection{The Diffusion Equation}
The Figure \ref{fig:diffusion} shows the solution for the Diffusion equation as described in equation \ref{eq:diffusion}. The figure depicts the spatial-temporal domain, where the x-axis represents the time($t$) and the y-axis represents the space($x$). In the first row we have the analytical high-fidelity solution, the second and third rows illustrate the solutions given by the PSO-PINN and the ADAM ensemble, respectively. Notably, the PSO-PINN obtained a better approximation to the original PDE, especially in the first half of the time dimension. The $L_2$ error found in the PSO-PINN solution was 6.54E-02, while the error for the ADAM ensemble was 1.05E-01. 

\begin{figure*}
\begin{center}
% \includegraphics[width=2\columnwidth]{fig/diffusion.png} % paper version
\includegraphics[width=1\columnwidth]{fig/diffusion.png} % arXiv version
\hfill
\end{center}
\caption{
% 
\textbf{Diffusion Equation} -- Results across the spatial-temporal domain. The first row represents the high-fidelity analytical solution. In the second row is the PSO-PINN solution, and in the third row the solution from a ensemble of traditional PINNs using ADAM as optimizer.
}
\label{fig:diffusion}
\end{figure*}


\subsubsection{The Allen-Cahn Equation}

The Allen-Cahn Equation (described in equation \ref{eq:allen-cahn}) is used here to illustrate the usage of supplementary data to solve a PDE. We previously created a dataset distributed over the domain 
$x \in [-1, 1]$, and $t \in [0, 1]$ and use it to give supplementary information for solving the problem. The purpose is to show that PSO-PINN framework incorporates well the data Loss ($\mathcal{L}_d$). The solutions for the problem are represented in Figure \ref{fig:allen-cahn}. We can see that both ensembles had good results, although the PSO-PINN reached general better precision.
When compared with an ensemble of traditional PINNs using ADAM optimization, we can notice that the PSO-PINN algorithm was able to reduce uncertainty in certain locations of the spatial-temporal domain. 




\begin{figure}
\begin{center}
\includegraphics[width=0.96\columnwidth]{fig/allen-cahn.png} 
\hfill
\end{center}
\caption{
% 
\textbf{Allen-Cahn Equation} --The result depicted as cross-sections above the spatial-temporal domain. The left column show the PSO-PINN solution and the right column show the solution for an ensemble of traditional PINNs optimized using ADAM.
}
\label{fig:allen-cahn}
\end{figure}

